Pointwise Mutual Information Based Metric and Decoding Strategy for Faithful Generation in Document Grounded Dialogs

A major concern in using deep learning based generative models for document-grounded dialogs is the potential generation of responses that are not \textit{faithful} to the underlying document. Existing automated metrics used for evaluating the faithfulness of response with respect to the grounding document measure the degree of similarity between the generated response and the document's content. However, these automated metrics are far from being well aligned with human judgments. Therefore, to improve the measurement of faithfulness, we propose a new metric that utilizes (Conditional) Point-wise Mutual Information (PMI) between the generated response and the source document, conditioned on the dialogue. PMI quantifies the extent to which the document influences the generated response -- with a higher PMI indicating a more faithful response. We build upon this idea to create a new decoding technique that incorporates PMI into the response generation process to predict more faithful responses. Our experiments on the BEGIN benchmark demonstrate an improved correlation of our metric with human evaluation. We also show that our decoding technique is effective in generating more faithful responses when compared to standard decoding techniques on a set of publicly available document-grounded dialog datasets.

==> pmi_decoding/sections/acknowledgements.tex <==
\section*{Acknowledgements}


==> pmi_decoding/sections/experiments_decoding_copy_20thJan1230.tex <==
\input{pmi_decoding/tables/decoding_performance}
\input{pmi_decoding/tables/human-eval}
\input{pmi_decoding/tables/subjective_analysis_examples}

\subsection{Evaluation of \pmidecodebold}
\label{sec:exp:decoding}
\noindent \textbf{Datasets:}
We work with three datasets for comparing the performance of  $\pmidecode$ against the likelihood based decoding strategy:
%We work with three datasets for PMI Decoding  Experiments
Multi-Doc2Dial~\cite{feng2021multidoc2dial}, Topical Chat\footnote{\url{https://github.com/alexa/Topical-Chat}}~\cite{Gopalakrishnan2019} and FaithDial\footnote{\url{https://huggingface.co/datasets/McGill-NLP/FaithDial}}~\cite{dziri&al22}. MultiDoc2Dial dataset contains dialogues that are goal-oriented and grounded on multiple documents. Topical Chat dataset consists of human-human conversations are grounded on documents and cover eight different subjects. The individuals involved in the conversation do not have specific roles assigned to them. FaithDial is a benchmark for evaluating dialogue systems where one participant, the information seeker, can ask a wide range of questions and the other participant, a bot wizard, can only provide information within a certain scope.
\input{pmi_decoding/tables/decoding_data_stats}

\noindent 
\textbf{Results:}
We finetune bart-large\footnote{\url{https://huggingface.co/facebook/bart-large}} using the code\footnote{\url{https://github.com/McGill-NLP/FaithDial}} made available by Dziri et al.~\shortcite{dziri&al22a} for all the three datasets in Table~\ref{tab:datasets}. Unless otherwise specified, the default parameter values are used. To fine-tune on Multi-Doc2dial, we employ a batch size of 16 for training, accumulate gradients for 4 steps, and train for 50 epochs with a patience of 20. We fine-tune FaithDial using 4 gradient accumulation steps for 10 epochs. For TopicalChat, we use a batch size of 16 for training and train for 10 epochs. For all the three datasets, we use the model checkpoint which returns the best perplexity score on the development set. Table ~\ref{tab:results} shows various faithfulness and relevance metrics computed for the test set for all the three datasets.

Using PMI decoding strategy (PMI, PMIEqWt and PMINoMask) improves all four faithfulness metrics compared to a greedy approach. We find that while PMINoMask has the highest faithfulness metrics, its relevance scores are the lowest. This can be explained by the fact that the response space of PMINoMask is not restricted. PMIEqWt generates better relevance scores for two out of three scores while taking a hit on the faitfulness metrics. PMI decoding strategy results in the best tradeoff between faithfulness and relevance. We thus use responses generated using PMI for human evaluation. We do notice that though PMI generates more faithful responses, the relevance scores seem to be lower than the greedy approach. We investigate this in detail in human evaluation.

\noindent \textbf{Human Evaluation:} We perform human evaluation experiments to compare (1) \textit{relevance} - the ability to generate responses that are contextually correct given the dialog history, (2) \textit{faithfulness} - the ability to generate responses that are faithful to the given document, and (2) \textit{grammar} --  ability to generate grammatically correct and fluent responses. All three dimensions were categorically labeled as agree, neutral, or disagree. We sampled 50 random (document, dialog history, response) tuples each from multidoc2dial and Topical Chat. We evaluate the responses generated by two decoding techniques: greedy and $\pmidecode$. We collected a total of 1800 labels from the judges.



The results are summarized in Table \ref{tab:human-eval}. For each dimension we report the percentage of responses that were rated \textit{agree}. As expected, \pmidecode\ generates more faithful responses compared to greedy. We observe a 15\% improvement in faithfulness compared to greedy decode on both the datasets.We observe that \pmidecode\ improves relevance on multi-doc2dial but slightly deteriorates on topical chat. 

As \pmidecode\ maximises not just the likelihood of responses, but a combination of likelihood and faithfulness, we expected the responses to contain grammatical error compared to greedy decode. To counter this issue, we proposed to use a weighted combination of likelihood and faithfulness during decode, with a higher weight on likelihood. We also restricted the vocabulary during each decode step to just the \textit{top-p} subset. We were glad to see that these mitigation techniques helped in reducing the grammatical mistakes made by \pmidecode. We see that the grammar is is only slightly inferior to greedy on both the datasets. 

Out of six in-house annotator, four were experts in dialog research and two were beginners. We use Fleiss Kappa \cite{Fleiss1973TheEO} to measure the inter-annotator agreement. We find the agreement is moderate (0.58) for relevance, substantial (0.63) for faithfulness, and almost perfect (0.9) for grammar. 

\noindent \textbf{Subjective Analysis:}


==> pmi_decoding/sections/methods_copy_17thJan.tex <==
\section{Background}
In this section, we first review the task of document-grounded dialog response generation, followed by a  definition of `faithfulness' of the generated response to the document given the dialogue history.
%We then define metric to compute faithfulness of generated responses with respect to the document.

\vspace{1.2ex}
\noindent
\textbf{Document Grounded Response Generation:}
Let dialog history $\history = [\utterance_1, \cdots \utterance_{\turnm}]$ be a sequence of $m$ utterances in the dialog so far and $\doc$ be the document on which the dialog is grounded. 
The task of  document--grounded dialog response generation
is to predict the next response, $\response = \responseseq{T}$, one token at a time, given the dialog history $\history$ and the document $\doc$. 
\ycom{
Here,  $\forall i, \responseword_i \in \vocab$, 
where $\vocab$ is the vocabulary of all possible tokens. 
The underlying model learns a probability distribution $\probof{}{\response | \doc,\history}$ over all possible responses $\response \in \vocab^+$. Typically, this distribution is factorized over the tokens of $\response$ as:
}
\begin{equation}
    \probof{}{\response | \doc,\history} = \prod_{\stept=1}^T \probof{}{\responseword_{\stept} | \doc,\history, \partialresponse{\stept-1}}
    \label{eq:response-generation}
\end{equation}

%Typically, the selection of the next word $\responseword_\stept$ from $\probof{}{\responseword_{\stept} | \doc,\history, \responseword_{1:\stept-1}}$ is guided by the underlying decoding strategies such as greedy or nucleus sampling. 

\vspace{1.2ex}
\noindent
\textbf{Faithfulness Metric:}
Unlike most of the existing definitions (and metrics) for faithfulness that focus mainly on document $\doc$ and response $\response$ but ignore $\history$ (maybe for the sake of uniformity across different tasks such as summarization, grounded dialogue generation \etc) \cite{dziri&al22a, dziri&al22}, we qualify the definition of faithfulness specifically for the task of document grounded dialogue generation.
Formally, a response $\response$ is considered `faithful' to a given document $\doc$ and the dialogue history $\history$ iff $\doc, \history \vDash \response$, where $\vDash$ represents logical entailment.

A faithfulness metric should quantify the faithfulness of the response $\response$ to the document $\doc$ and dialogue history $\history$. 
In general, such a metric should take $\response, \doc$ and $\history$ as its input and compute a score, $\faithfulnessmetric(\response, \doc, \history) \in \realspace$, such that a higher value of $\faithfulnessmetric(\response, \doc, \history)$ indicates a more faithful response. 

\begin{comment}

\section{Background}

\textbf{Document-Grounded dialogue generation:}
Let 
dialogue context $\history = [\utterance_0 \cdots \utterance_{\turnm-1}]$ be a sequence of utterances between a user and a model $\model$, which is typically a fine-tuned Large Language Model such as GPT2 \cite{}, BLOOM \cite{}.
Based on $\history$ and a given document $\doc$, the task for the model $\model$ at turn $\turnm$ is to generate a response $\response$
that is grounded in the document $\doc$ and forms the next utterance $\utterance_{\turnm}$ in the dialogue context.
Notice that the response $\response$ consists of a sequence of tokens selected from a vocabulary $\vocab$. 
We use $\response[\stept]$ and upper--case $\responsevariable[\stept]$ to represent the token and the corresponding random variable (respectively) at step $\stept$ of generation.
At each step $\stept$ during generation,
%of response $\response$, 
model $\model$ first outputs a conditional probability distribution,  $\probof{\responsevariable[\stept]}{\token | \doc,\history,\response[:(\stept-1)]}$, with $\token \in \vocab$, conditioned on the document $\doc$, history $\history$, and the response $\response[:(\stept-1)]$ generated till $\stept$.
%Here $\responsevariable[\stept]$ corresponds to the discrete random variable whose value, selected from vocabulary $\vocab$, determines the token $\response[\stept]$ generated at $\stept$.
Typically, this selection of the next token is based on an appropriate decoding strategy such as greedy or nucleus sampling \cite{}.

Further, let $\faithfulnessmetric(\response, \doc, \history) \in \realspace$ be a metric that quantifies the `faithfulness' of response $\response$ to the document $\doc$ given context $\history$.
A higher value of $\faithfulnessmetric(\response, \doc, \history)$ indicates a more faithful response. 
In the next section, we first introduce a new metric for faithfulness based on the information theoretic concept of Point--wise Mutual Information. 
Then, based on our metric, we propose a novel decoding strategy with the objective of generating more faithful responses as compared to greedy or nucleus sampling. 

\end{comment}

\section{Approach}

In this section, we describe our proposed metric for faithfulness based on the information theoretic concept of Point--wise Mutual Information. We then we propose a novel decoding strategy based on our metric, with the objective of generating more faithful responses as compared to greedy or nucleus sampling. 

\subsection{PMI as a Faithfulness Metric}

%\noindent \textbf{Point--wise Mutual Information:}
Let $\randvariablea$ and $\randvariableb$ represent two discrete random variables over discrete space $\spacea$ and $\spaceb$ respectively. 
Further, let $\randvaluea \in \spacea$ and $\randvalueb \in \spaceb$ represent their possible outcomes respectively.
In a little abuse of notation, we use function $\discreteprob()$ to represent an appropriate probability or conditional probability distribution function.
Then, Mutual Information between $\randvariablea$ and $\randvariableb$  captures the amount of information overlap between them, and is defined as expectation over Point--wise Mutual Information:
\begin{align*}
    \mi(\randvariablea; \randvariableb) =
    \sum\limits_{\randvaluea \in \spacea; \randvalueb \in \spaceb}
    \discreteprob(\randvaluea, \randvalueb)
    &\pmi(\randvaluea; \randvalueb)  \text{  where  } \\
    \pmi(\randvaluea; \randvalueb) 
    = 
    \log \frac{\discreteprob(\randvaluea, \randvalueb)}
              {\discreteprob(\randvaluea) \discreteprob(\randvalueb)} 
    =& \log \frac{\discreteprob(\randvalueb)\discreteprob(\randvaluea | \randvalueb)}
    {\discreteprob(\randvaluea) \discreteprob(\randvalueb)} \\
    =& \log \frac{\discreteprob(\randvaluea | \randvalueb)}
    {\discreteprob(\randvaluea)}
\end{align*}

Now, if $\randvariablec$ is another random variable, with $\randvaluec \in \spacec$ representing its possible outcome, one can define Conditional Point--wise Mutual Information (CPMI) between $\randvaluea$ and $\randvalueb$ given $\randvaluec$ as:
\begin{equation*}
    \cpmi(\randvaluea; \randvalueb | \randvaluec) = 
    \log \frac{\discreteprob(\randvaluea, \randvalueb | \randvaluec)}
              {\discreteprob(\randvaluea | \randvaluec) \discreteprob(\randvalueb |\randvaluec)}
              = 
    \log \frac{\discreteprob(\randvaluea | \randvalueb, \randvaluec)}
    {\discreteprob(\randvaluea | \randvaluec)}
\end{equation*}

We use the notion of  CPMI between generated response $\response$ and the document $\doc$ given the context $\history$ to capture the influence of the document in generating the response. 
We define our metric, $\pmimetric$, for faithfulness of the response $\response$ to the document $\doc$ as:
\begin{align}
    &\pmimetric(\response; \doc | \history) =
    \log \frac
    {\condprobfn{\response, \doc}{\history}}
    {\condprobfn{\response}{\history} \condprobfn{\doc}{\history}} = \\
    &=
    \log \frac
    {\condprobfn{\doc}{\history} \condprobfn{\response}{\doc,\history}}
    {\condprobfn{\response}{\history} \condprobfn{\doc}{\history}}
    =
    \log \frac
    {\condprobfn{\response}{\doc,\history}}
    {\condprobfn{\response}{\history}} 
\end{align}

Measuring $\pmimetric$ requires computing
the conditional probability of generating the response given the document and history (numerator) and 
the conditional probability of generating the response given only the current context (denominator).
%Intuitively, it captures the influence of the given document on generating the response.
We use a pre-trained language model, such as BLOOM \cite{} or GPT2 \cite{}, to compute these conditional probabilities.
For the remainder of the paper, we would use the term `CPMI of response $\response$ given context $\history$' to implicitly mean CPMI between response $\response$ and document $\doc$ conditioned on the context $\history$. 

\subsection{PMI based Decoding Strategy}
\ycom{Need to change the pitch to make it consistent with introduction. \\
1. Start with the overall objective of selecting a response that is both likely and faithful. \\
2. Describe the naive bruteforce method that is intractable. Namely, generate all possible responses and pick the one with highest combined score. \\
3. Describe the alternative of greedy approach that maximizes faithfulness of the partially generated response at each step. This is same as replacing $\pmimetric$ in eqn 5 with general function F.\\
4. Then show that using q2 or other metrics will make it difficult. \\
5. And then finally argue that when F is pmifaith,  it becomes tractable!
}

Once the model has been fine-tuned, we typically select a response that has maximum log likelihood:
\begin{equation*}
    \response = \argmax\limits_{\tilde{\response} \in \vocab^+}
    \log \probof{}{\tilde{\response} | \doc, \history}
\end{equation*}
Our objective instead is to select a response that has a high likelihood and is also faithful to the given document and dialogue history.
This can be achieved by 
%selecting a response that 
maximizing not just the likelihood, but a scoring function combining both likelihood and faithfulness quantified using an appropriate metric $\faithfulnessmetric$. With $\alpha \in [0,1]$, $\mybeta = 1 - \alpha$, and a linear scoring function, we get:
\begin{align*}
    \response =& \argmax\limits_{\tilde{\response} \in \vocab^+} \score(\tilde{\response},\doc,\history) \text{, where,  } \\
    \score(\tilde{\response},\doc,\history) =& \mybeta\log \probof{}{\tilde{\response} | \doc, \history} + 
    \alpha\faithfulnessmetric(\tilde{\response},\doc,\history)
\end{align*}
When using an auto--regressive model that factorizes the probability distribution and generates the response one token at a time, typically a decoding strategy is used. For example, greedy decoding would sample the next token $\responseword_{\stept}$ such that it maximizes the overall score of the partial response $\responseseq{\stept}$:
\begin{align}
\responseword_{\stept} = \argmax\limits_{\token \in \vocab}{}&
 \score(\responseseqwithvar{\stept-1}{\token},\doc,\history) \\
\begin{split}
= \argmax\limits_{\token \in \vocab}{}&
\mybeta\log \probof{}{\responseseqwithvar{\stept-1}{\token} | \doc, \history}\\
{}& + \alpha\faithfulnessmetric(\responseseqwithvar{\stept-1}{\token}, \doc, \history)
\end{split} \\
\begin{split}
    = \argmax\limits_{\token \in \vocab}{}&
\mybeta[\log \probof{}{\responseseq{\stept-1} | \doc, \history}\\
{}& + \log\probof{}{\token| \doc, \history,\partialresponse{\stept-1}}] \\
{}& +\alpha\faithfulnessmetric(\responseseqwithvar{\stept-1}{\token}, \doc, \history)
\end{split} \\
\begin{split}
    = \argmax\limits_{\token \in \vocab}{}&
\mybeta\log \probof{}{\token| \doc, \history, \partialresponse{\stept-1}}\\
{}& +\alpha\faithfulnessmetric(\responseseqwithvar{\stept-1}{\token}, \doc, \history)
\end{split}
\end{align}
In the above equations, the likelihood term has been factorized. Now, when we use metrics like \qtwo\ or BLEU as the faithfulness metric,
computing $\faithfulnessmetric$ for $|\vocab|$ possible partial responses at each step $\stept$ becomes computationally challenging.
On the other hand, when using $\pmimetric$ as our measure of faithfulness, we get:



At each step $\stept$ during generation of response $\response$, 
the model first outputs a conditional probability distribution,  %$\condprobfn{\responsevariable[\stept]}{\doc,\history,\response[:(\stept-1)]}$ 
$\probof{}{\token | \doc,\history,\partialresponse{\stept-1}}, \token \in \vocab$,  
which is conditioned on the document, dialogue context and the response generated till now.


Once the model has been fine-tuned, 
we use a decoding strategy to generate the response for a given document and context history.
At each step $\stept$ during generation of response $\response$, 
the model first outputs a conditional probability distribution,  %$\condprobfn{\responsevariable[\stept]}{\doc,\history,\response[:(\stept-1)]}$ 
$\probof{}{\token | \doc,\history,\partialresponse{\stept-1}}, \token \in \vocab$,  
which is conditioned on the document, dialogue context and the response generated till now.
%with $\token \in \vocab$. 
In the greedy decoding, the next token $\responseword_\stept$ is selected as:
\begin{equation*}
\responseword_{\stept} = \argmax\limits_{\token \in \vocab} \log \probof{}{\token | \doc,\history,\partialresponse{\stept-1}} 
\end{equation*}
While computing faithfulness, we measured CPMI between the response and document after the entire response has been generated.
Instead, at each generation step $\stept$, one can compute CPMI between the partial response generated till now ($\response[:(\stept-1)]$) and the document $\doc$.
Now the selection of the next token can be made to 
maximize not just the probability, but a convex sum of probability and CPMI of partial response after step $\stept$.
%and the document $\doc$.
Formally, we define a score function, $\score_{\stept}(\token), \token \in \vocab$, whose maxima determines the next token:
\begin{align}
\response[\stept] &= {} \argmax_{\token \in \vocab} \score_{\stept}(\token) \text{   where  } \label{eq:argmaxscore} \\
\begin{split}\label{eq:score}
    \score_{\stept}(\token) &= {}
    \alpha \pmimetric(\concat{\response[:(\stept-1)]}{\token} ; \doc | \history) + \\
    & (1-\alpha)\log \probof{\responsevariable[\stept]}{\token | \doc,\history,\response[:(\stept-1)]} 
    \end{split}
\end{align}
Here, $\concat{\response[:(\stept-1)]}{\token}$ is the concatenation of token $\token$ to the existing partial response and represents the partial response after step $\stept$ if $\token$ is selected at $\stept$.
Interestingly, one can decompose the $\pmimetric$ of partial response ($\response[:\stept]$) after step $\stept$ into sum of $\pmimetric$ of partial response ($\response[:(\stept-1)]$) before step $\stept$, and CPMI between the token $\response[\stept]$ and document $\doc$ conditioned on not just the context $\history$ but also the partial response $\response[:(\stept-1)]$: 
\begin{align}
    \pmimetric&(\response[:\stept] ; \doc | \history) =
    \log \frac{\condprobfn{\response[:\stept]}{\doc,\history}}
             {\condprobfn{\response[:\stept]}{\history}} \\
    \begin{split}
     = {} & \log \frac{\condprobfn{\response[:(\stept-1)]}{\doc,\history}}
             {\condprobfn{\response[:(\stept-1)]}{\history}} 
        + \\
     {} &  \log  \frac{\condprobfn{\response[\stept]}{\doc,\history,\response[:(\stept-1)]}}
             {\condprobfn{\response[\stept]}{\history, \response[:(\stept-1)]}}                 
    \end{split} \\
    \begin{split}
    \label{eq:pmibreakup}
     = {} & \pmimetric(\response[:(\stept-1)]; \doc | \history)
        + \\
        {} & \cpmi(\response[\stept];\doc | \history, \response[:(\stept-1)])
    \end{split}
\end{align}
Using \cref{eq:pmibreakup} in \cref{eq:score}, we get:
\begin{equation}
\label{eq:scorebreakup}
\begin{split}
    \score_{\stept}(\token) = 
    \alpha 
    & \pmimetric(\response[:(\stept-1)] ; \doc | \history) + \\
    \alpha & \cpmi(\token;\doc | \history, \response[:(\stept-1)])
      + \\
    (1-\alpha) & \log \probof{\responsevariable[\stept]}{\token | \doc,\history,\response[:(\stept-1)]} 
    \end{split}
\end{equation}
Now notice that the first term in \cref{eq:scorebreakup} is independent of $\token$ and hence it can be dropped while taking the $\argmax$ in \cref{eq:argmaxscore} 
Also, to measure the required CPMI in \cref{eq:scorebreakup}, %between token $\token$ and document $\doc$ given context $\history$ and partial response $\response[:(\stept-1)]$,
we can use the language model $\model$ to compute the conditional probabilities $\probof{\responsevariable[\stept]}{\token | \doc, \history, \response[:(\stept-1)]}$ (numerator) and
$\probof{\responsevariable[\stept]}{\token | \history, \response[:(\stept-1)]}$ (denominator) by separately passing $\doc$,$\history$, $\response[:(\stept-1)]$ and $\history$, $\response[:(\stept-1)]$, respectively, through model $\model$.
Therefore, we get:
\begin{align}
    \response[\stept] = & \argmax\limits_{\token \in \vocab} \score_{\stept}(\token) \\
    = & \argmax\limits_{\token \in \vocab} \score'_{\stept}(\token) \text{  where  } \\
    \begin{split}
    \score'_{\stept}(\token) = &
    \alpha \log \frac{\probof{\responsevariable[\stept]}{\token | \doc, \history, \response[:(\stept-1)]}}{\probof{\responsevariable[\stept]}{\token | \history, \response[:(\stept-1)]}} + \\
    (1-&\alpha)  \log \probof{\responsevariable[\stept]}{\token | \doc, \history, \response[:(\stept-1)]}
    \end{split}
\end{align}

In the next section, we first validate the ability of our metric, $\pmimetric$, to identify faithful responses and then demonstrate that our novel decoding strategy indeed generates more faithful responses than greedy decoding based on just probability.


\begin{comment}
\begin{align}
    \response[{\stept}] =& \argmax\limits_{\token \in \vocab} 
    \score(\token) \text{   where   }  \\
    \score(\token) =& 
    \alpha \log \frac{\probof{\responsevariable[\stept]}{\token | \doc,\history,\response[:(\stept-1)]}}
                     {\probof{\responsevariable[\stept]}{\token | \history,\response[:(\stept-1)]}}
    + 
    (1-\alpha) \log \probof{\responsevariable[\stept]}{\token | \doc,\history,\response[:(\stept-1)]} 
\end{align}
\end{comment}

==> pmi_decoding/sections/related_works.tex <==
\section{Related Works}
%Our research has two significant contributions: $\pmimetric$, a metric to quantify faithfulness in document--grounded dialogue systems, and $\pmidecode$, a novel decoding strategy to mitigate hallucination by generating faithful responses.
In this section, we discuss related works in the areas of quantifying faithfulness and mitigating hallucination in document--grounded dialogue systems.
%We use the term `faithfulness' to indicate lack of `hallucination'.

\noindent \textbf{Faithfulness:}
%Different researchers have used various but related terms to define and quantify faithfulness of a system's output to a given information source in various generation tasks such as summarization, paraphrasing, knowledge grounded dialogues. \citet{cao&al18,chen7&al21, dziri&al22a,rashkin&al21b} use the term faithfulness; \citet{cao&al20, cao&wang21, wu&al21, honovich&al21,kryscinski&al20,santhanam&al21} use factual consistency; \citet{goodrich&al19,alambo&al22} use factual accuracy; \cite{chen&al20, chen&al20a, sipos&al12} use fidelity; \citet{dziri&al22,rashkin&al21a} use attribution, and finally \cite{xiao&wang21,filippova20, zhou&al21,shuster&al21, dziri&al21} use `hallucination' to denote the lack of faithfulness. Although various terms are used, the idea behind it is the same, which is the extent to which the generated response aligns with the available knowledge.
%Different researchers have used various but related terms to define and quantify faithfulness of a system's output to a given information source in various generation tasks such as summarization, paraphrasing, knowledge grounded dialogues. \citet{cao&al18,chen&al21} use the term faithfulness; \citet{cao&al20, cao&wang21, wu&al21} use factual consistency; \citet{goodrich&al19,alambo&al22} use factual accuracy; \cite{chen&al20, chen&al20a, sipos&al12} use fidelity; \citet{rashkin&al21a} use attribution, and finally \cite{xiao&wang21, zhou&al21,shuster&al21, dziri&al21} use `hallucination' to denote the lack of faithfulness. Although various terms are used, the idea behind it is the same, which is the extent to which the generated response aligns with the available knowledge.
Researchers have used various terms such as faithfulness \cite{cao&al18}, factual consistency \cite{cao&al20,santhanam&al21}, factual accuracy \cite{goodrich&al19}, fidelity \cite{chen&al20}, attribution \cite{rashkin&al21a} and hallucination (i.e., the lack of faithfulness) \cite{xiao&wang21} to define and quantify faithfulness of a model's generated text to a given knowledge.
%knowledge intensive NLP Tasks.


Most of the works focusing on evaluating faithfulness propose to train a classifier for the task \cite{goodrich&al19,kryscinski&al20,dziri&al22a}. Whereas our proposed metric doesn't require any training and is agnostic to the underlying data.
%In a recent work, \citet{dziri&al22a} fine-tune a RoBERTa based classifier to predict faithfulness in knowledge grounded dialogue systems. We compare it against our metric $\pmimetric$ that doesn't require any training and is agnostic to the underlying dataset.
%Most of the works focusing on evaluating faithfulness propose to train a classifier for the task. \todo{we can keep just the first line and cite all works there.} \citet{goodrich&al19} train a relation classifier, and  \citet{kryscinski&al20} fine--tune a BERT based classifier using weak supervision to predict factual accuracy in summarization task. In a recent work, \citet{dziri&al22a} fine-tune a RoBERTa based classifier, to predict faithfulness in knowledge grounded dialogue systems. They call their classifier \textit{faithcritic} and make it publicly available. In our experiments, we compare it against our metric $\pmimetric$ that doesn't require any training and is agnostic to the underlying dataset.
Recently, \citet{honovich&al21} proposed \qtwo\ for quantifying faithfulness. It uses a question generator to first generate question--answer (QA) pairs from the generated response. Then a QA system is used to find an answer, to the generated question, from the document. Finally, an NLI system is used to compare the two answers. %Unlike \citet{scialom&al21}, they use an NLI system to quantify faithfulness by comparing the two answers.
Though \qtwo\ uses the given document to check the faithfulness of a response, it ignores the dialog history. Thus, it may fail at handling non--sentential responses as depicted in \cref{fig:intro}. Our metric $\pmimetric$ addresses this issue.

\vspace{0.1ex}
\noindent\textbf{Mitigating Hallucination:}
Hallucination can be reduced by pre--processing data and removing instances from training data that are factually incorrect~\cite{shen&al21}. It can also be reduced by training control tokens and using them during response generation~\cite{filippova20,rashkin&al21b}. 
We focus on decoding and do not require explicit changes to the training procedure or data.

%\cite{gabriel&al21} propose a generator--discriminator framework to generate faithful summaries by training the discriminator to re--rank different summaries based on faithfulness.

In addition to the above two areas, many recent works \cite{dziri&al22, honovich&al22} have released different benchmarks that can be used to evaluate the performance of faithfulness metrics. 
While \citeauthor{honovich&al22} aim to standardize benchmark datasets across different generation tasks, \citeauthor{dziri&al22} focus on document--grounded dialogues, and thus we use it to compare our metric with various baselines. Finally, \citet{ji&al22} presents a survey that discusses hallucination in various natural language generation tasks, including document--grounded dialogue response generation.


%The advancements in sequence-to-sequence deep learning technologies, such as Transformer-based language models, have significantly increased the capabilities of Natural Language Generation (NLG) in recent years. The improvement in natural language generation has resulted in more fluent and logical output, aiding in the development of related tasks such as summarization, dialogue creation, and text generation from data. However, it should also be noted that deep learning-based generation can produce \textbf{hallucinated text}, negatively impacting system performance and failing to meet user expectations in practical situations ~\cite{ji&al22}. Thus, recently there has been lot of interest in addressing the problem of hallucination: by formally defining, quantifying and mitigating it while generating responses.

%Different researchers have used various but related terms to define hallucination in the context of dialog systems. \cite{cao&al18,zhou&al21,chen7&al21,filippova20, xiao&wang21, dziri&al22a, rashkin&al21} use faithfulness, \cite{cao&al20,cao&wang21, wu&al21, honovich&al21} use factual consistency, \cite{chen&al20,chen&al20a,sipos&al12} use fidelity, \cite{dziri&al22,rashkin&al21} use attribution, or \cite{shuster&al21, dziri&al21} use `hallucination' to denote the lack of faithfulness. Although various terms are used, the idea behind it is the same, which is the extent to which the generated response aligns with the available knowledge.

% Given that the research is in its nascent stages, different researchers have used different but related terminology for defining the phenomenon where the generated response can or can not be grounded/verified on the given knowledge. For example, \cite{cao&al18,zhou&al21,chen7&al21,filippova20, xiao&wang21, dziri&al22a, rashkin&al21} use faithfulness, \cite{cao&al20,cao&wang21, wu&al21, honovich&al21} use factual consistency, \cite{chen&al20,chen&al20a,sipos&al12} use fidelity, \cite{dziri&al22,rashkin&al21} use attribution, or \cite{shuster&al21, dziri&al21} use `hallucination' to denote the lack of faithfulness.
% Despite these different terms, the underlying concept is related, and refers to the degree to which the generated response can be grounded or verified with respect to the given knowledge.

% 3. \citet{ji&al22} presents a survey of many recent works that focus on quantifying and mitigating hallucination in various natural language generation tasks, including content grounded dialogue systems.

% 1. Cliched line about issue of hallucination being amplified by llms, recent acceleration in the research of llms and their subsequent application for various natural language generation tasks has brought the attention of researchers to the task of quantifying and mitigating hallucination. 

%There has been a large body of work for quantifying faithfulness~\cite{ji&al22}. In this work, we will focus on the task of document grounded dialog systems. $Q^{2}$~\cite{honovich&al21} uses natural language inference (NLI) to determine the accuracy of answers by asking and answering questions. Though $Q^{2}$ uses document to check the faithfulness of a response, it does not make uses of the conversation context. Thus it may fail at handling non-sentential responses as depicted in Figure~\ref{fig:intro}. Our proposed metric PMI-Faith addresses this issue.



% \textbf{Quantifying Hallucination/Faithfulness:}

==> pmi_decoding/sections/related_works_20thJan9pm.tex <==
\section{Related Works}
Our research has two significant contributions: the development of a new faithfulness metric called PMI-Faith, which can be used to measure the faithfulness of responses in document-grounded dialogue, and a new decoding method that utilizes PMI-Faith to generate more faithful responses and mitigate hallucination. Therefore, we will focus on related work in these two areas.
\cite{ji&al22} presents a survey of many recent works that focus on quantifying and mitigating hallucination in various natural language generation tasks, including document grounded dialogue systems, which is the main focus area of this paper.  
We use the term `faithfulness' to indicate lack of `hallucination'.

\textbf{Faithfulness metrics:}
Different researchers have used various but related terms to define and quantify faithfulness in the context of dialog systems. \citet{cao&al18,zhou&al21,chen7&al21,filippova20, xiao&wang21, dziri&al22a, rashkin&al21} use the term faithfulness, \citet{cao&al20,cao&wang21, wu&al21, honovich&al21} use factual consistency, \cite{chen&al20,chen&al20a,sipos&al12} use fidelity, \cite{dziri&al22,rashkin&al21} use attribution, and \cite{shuster&al21, dziri&al21} use `hallucination' to denote the lack of faithfulness. Although various terms are used, the idea behind it is the same, which is the extent to which the generated response aligns with the available knowledge.

$Q^{2}$~\cite{honovich&al21} uses natural language inference (NLI) to determine the accuracy of answers by asking and answering questions. Though $Q^{2}$ uses document to check the faithfulness of a response, it does not make uses of the conversation context. Thus it may fail at handling non-sentential responses as depicted in \cref{fig:intro}. Our proposed metric PMI-Faith addresses this issue.

\textbf{Mitigating Hallucination:}
Hallucination can be reduced by pre-processing data and remove instances from training which are factually incorrect~\cite{Shen2021IdentifyingUS}. Adding learnt control tokens can also be used to reduce hallucination while generating responses ~\cite{rashkin&al21}. Our work does not require learning any control tokens or removing an existing data from training.


%The advancements in sequence-to-sequence deep learning technologies, such as Transformer-based language models, have significantly increased the capabilities of Natural Language Generation (NLG) in recent years. The improvement in natural language generation has resulted in more fluent and logical output, aiding in the development of related tasks such as summarization, dialogue creation, and text generation from data. However, it should also be noted that deep learning-based generation can produce \textbf{hallucinated text}, negatively impacting system performance and failing to meet user expectations in practical situations ~\cite{ji&al22}. Thus, recently there has been lot of interest in addressing the problem of hallucination: by formally defining, quantifying and mitigating it while generating responses.

%Different researchers have used various but related terms to define hallucination in the context of dialog systems. \cite{cao&al18,zhou&al21,chen7&al21,filippova20, xiao&wang21, dziri&al22a, rashkin&al21} use faithfulness, \cite{cao&al20,cao&wang21, wu&al21, honovich&al21} use factual consistency, \cite{chen&al20,chen&al20a,sipos&al12} use fidelity, \cite{dziri&al22,rashkin&al21} use attribution, or \cite{shuster&al21, dziri&al21} use `hallucination' to denote the lack of faithfulness. Although various terms are used, the idea behind it is the same, which is the extent to which the generated response aligns with the available knowledge.

% Given that the research is in its nascent stages, different researchers have used different but related terminology for defining the phenomenon where the generated response can or can not be grounded/verified on the given knowledge. For example, \cite{cao&al18,zhou&al21,chen7&al21,filippova20, xiao&wang21, dziri&al22a, rashkin&al21} use faithfulness, \cite{cao&al20,cao&wang21, wu&al21, honovich&al21} use factual consistency, \cite{chen&al20,chen&al20a,sipos&al12} use fidelity, \cite{dziri&al22,rashkin&al21} use attribution, or \cite{shuster&al21, dziri&al21} use `hallucination' to denote the lack of faithfulness.
% Despite these different terms, the underlying concept is related, and refers to the degree to which the generated response can be grounded or verified with respect to the given knowledge.

% 3. \citet{ji&al22} presents a survey of many recent works that focus on quantifying and mitigating hallucination in various natural language generation tasks, including content grounded dialogue systems.

% 1. Cliched line about issue of hallucination being amplified by llms, recent acceleration in the research of llms and their subsequent application for various natural language generation tasks has brought the attention of researchers to the task of quantifying and mitigating hallucination. 

%There has been a large body of work for quantifying faithfulness~\cite{ji&al22}. In this work, we will focus on the task of document grounded dialog systems. $Q^{2}$~\cite{honovich&al21} uses natural language inference (NLI) to determine the accuracy of answers by asking and answering questions. Though $Q^{2}$ uses document to check the faithfulness of a response, it does not make uses of the conversation context. Thus it may fail at handling non-sentential responses as depicted in Figure~\ref{fig:intro}. Our proposed metric PMI-Faith addresses this issue.



% \textbf{Quantifying Hallucination/Faithfulness:}

==> pmi_decoding/tables/decoding_grid_backup17Oct2023.tex <==

\begin{table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}|l|cccc|cccc|@{}}
\hline
 &
  \multicolumn{4}{c|}{\textbf{PMIF}} &
  \multicolumn{4}{c|}{\textbf{RougeL}} \\ \hline
\diagbox{$p$}{$\alpha$} &
  {\textbf{0}} &
  {\textbf{0.25}} &
  {\textbf{0.5}} &
  \textbf{1} &
  {\textbf{0}} &
  {\textbf{0.25}} &
  {\textbf{0.5}} &
  \textbf{1} \\ \hline
\textbf{0.6} &
  \cellcolor{grayl}{0.52} &
  \cellcolor{grayl}{0.58} &
  {0.59} &
  0.59 &
  \cellcolor{grayl}{0.40} &
  \cellcolor{grayl}{0.40} &
  {0.39} &
  0.38 \\ 
\textbf{0.75} &
  \cellcolor{grayl}{0.52} &
  {0.60} &
  {0.61} &
  0.60 &
  \cellcolor{grayl}{0.40} &
  {0.39} &
  {0.38} &
  0.36 \\ 
\textbf{0.9} &
  \cellcolor{grayl}{0.52} &
  {0.61} &
  {0.62} &
  0.57 &
  \cellcolor{grayl}{0.40} &
  {0.39} &
  {0.36} &
  0.30 \\ 
\textbf{1} &
  \cellcolor{grayl}{0.52} &
  {0.61} &
  {0.56} &
  \cellcolor{pink}0.34 &
  \cellcolor{grayl}{0.40} &
  {0.38} &
  {0.30} &
  \cellcolor{pink}0.05 \\ \hline
\end{tabular}%
}
\caption{ \label{tab:grid} Faithfulness and relevance of the responses generated by beam sampling using different configurations of $\alpha$ and $top-p$ masking on the FaithDial dataset}.
\end{table}

==> pmi_decoding/tables/metric_performance_datasetwise.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
%\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l|rrrr@{}}
\toprule
\textbf{Metric} & \multicolumn{1}{c}{\textbf{CMU}} & \multicolumn{1}{c}{\textbf{TC}} & \multicolumn{1}{c}{\textbf{WoW}} & \multicolumn{1}{c}{\textbf{All}} \\ \midrule
Unigram F1   & 0.462          & 0.429          & 0.587          & 0.531          \\
SacreBLEU    & 0.027          & 0.000          & 0.620          & 0.479          \\
ROUGEL       & 0.140          & 0.050          & 0.647          & 0.518          \\
BERTScore    & 0.294          & 0.432          & 0.612          & 0.546          \\
faithcritic  & 0.156          & 0.039          & \textbf{0.794} & 0.573          \\
\qtwo\       & 0.543          & 0.487          & 0.705          & 0.610          \\
$\pmimetric$ & \textbf{0.663} & \textbf{0.584} & 0.771          & \textbf{0.697} \\ \bottomrule
\end{tabular}
%}
\caption{F1 Score of various metrics on each of the three datasets: CMU--DoG (CMU), Topical Chat (TC), and Wizards of Wikipedia (WoW)}
\label{tab:metric:datasetwise}
\end{table}
